Approximation Algorithms for LCS and LIS with Truly Improved Running Times

Longest common subsequence ($\mathsf{LCS}$) is a classic and central problem in combinatorial optimization. While $\mathsf{LCS}$ admits a quadratic time solution, recent evidence suggests that solving the problem may be impossible in truly subquadratic time. A special case of $\mathsf{LCS}$ wherein each character appears at most once in every string is equivalent to the longest increasing subsequence problem ($\mathsf{LIS}$) which can be solved in quasilinear time. In this work, we present novel algorithms for approximating $\mathsf{LCS}$ in truly subquadratic time and $\mathsf{LIS}$ in truly sublinear time. Our approximation factors depend on the ratio of the optimal solution size over the input size. We denote this ratio by $\lambda$ and obtain the following results for $\mathsf{LCS}$ and $\mathsf{LIS}$ without any prior knowledge of $\lambda$. $\bullet$ A truly subquadratic time algorithm for $\mathsf{LCS}$ with approximation factor $\Omega(\lambda^3)$. $\bullet$A truly sublinear time algorithm for $\mathsf{LIS}$ with approximation factor $\Omega(\lambda^3)$. Triangle inequality was recently used by [Boroujeni, Ehsani, Ghodsi, HajiAghayi and Seddighin SODA 2018] and [Charkraborty, Das, Goldenberg, Koucky and Saks FOCS 2018] to present new approximation algorithms for edit distance. Our techniques for $\mathsf{LCS}$ extend the notion of triangle inequality to non-metric settings.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Approximation Algorithms for LCS and LIS}{Rubinstein \textit{et al.}}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Approximation Algorithms for LCS and LIS with Truly Improved Running Times\thanks{Submitted to the editors DATE.}\thanks{A preliminary version of this work is appeared in FOCS'19}}

% Authors: full names plus addresses.
\author{Aviad Rubinstein\thanks{Stanford University, Stanford, CA 
  (\email{aviad@stanford.edu}, \url{https://cs.stanford.edu/~aviad/}).}
\and Saeed Seddighin\thanks{Toyota Technological Institute at Chicago, Chicago, IL 
  (\email{saeedreza.seddighin@gmail.com}, \url{https://sites.google.com/view/saeedrezaseddighin}).}
\and Zhao Song\thanks{Institute for Advanced Study, Princeton, NJ 
	(\email{magic.linuxkde@gmail.com }, \url{https://www.ias.edu/scholars/zhao-song}).}
\and Xiaorui Sun\thanks{University of Illinois, Chicago, IL 
	(\email{xiaorui@uic.edu}, \url{https://www.cs.uic.edu/~xiaorui/}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

